Observatory science with eXTP

In this White Paper we present the potential of the enhanced X-ray Timing and Polarimetry (eXTP) mission for studies related to Observatory Science targets. These include flaring stars, supernova remnants, accreting white dwarfs, low and high mass X-ray binaries, radio quiet and radio loud active galactic nuclei, tidal disruption events, and gamma-ray bursts. eXTP will be excellently suited to study one common aspect of these objects: their often transient nature. Developed by an international Consortium led by the Institute of High Energy Physics of the Chinese Academy of Science, the eXTP mission is expected to be launched in the mid 2020s.

==> dotar <==
tar cvf eXTP_WP_OS.tar \
2017SCGE.cls                    \
BB_1mCrab_ld_del_eemo_jz.eps	\
Clump.eps			\
collision.eps			\
dotar				\
elavsky4.png			\
eXTP_CV_fig.eps			\
extp.eps			\
eXTP_WP_OS.tex		\
facilities_vs9jan2018.pdf	\
famps_extp7.eps			\
figgrb1_vs6.eps			\
figgrb2b.pdf			\
figgrb3_vs3.eps			\
figgrbiron1_vs2.eps		\
figgrbiron2_vs2.eps		\
FoV_vs26092017.pdf		\
jean4m2.pdf			\
lc_extp5.eps			\
lmxb_orbitsn.pdf		\
LOFT_AGN_var_totcounts.pdf	\
patruno.png			\
radiomap3.eps			\
sens.pdf			\
snr1.eps			\
spectra.eps			\
stellarflare_artist.eps		\
v0332_crit.pdf                  \
wu2010.png                      \
picins.sty                      \
Print-CrossMark.eps                  \
Print-CrossMark-eps-converted-to.pdf \
figDrake3b.eps                       \
sn1006_1_srcut_sfa_1e4.eps           \
eXTP_WP_OS.pdf

gzip eXTP_WP_OS.tar

